NI-Tex: Non-isometric Image-based Garment Texture Generation

Existing industrial 3D garment meshes already cover most real-world clothing geometries, yet their texture diversity remains limited. To acquire more realistic textures, generative methods are often used to extract Physically-based Rendering (PBR) textures and materials from large collections of wild images and project them back onto garment meshes. However, most image-conditioned texture generation approaches require strict topological consistency between the input image and the input 3D mesh, or rely on accurate mesh deformation to match to the image poses, which significantly constrains the texture generation quality and flexibility. To address the challenging problem of non-isometric image-based garment texture generation, we construct 3D Garment Videos, a physically simulated, garment-centric dataset that provides consistent geometry and material supervision across diverse deformations, enabling robust cross-pose texture learning. We further employ Nano Banana for high-quality non-isometric image editing, achieving reliable cross-topology texture generation between non-isometric image-geometry pairs. Finally, we propose an iterative baking method via uncertainty-guided view selection and reweighting that fuses multi-view predictions into seamless, production-ready PBR textures. Through extensive experiments, we demonstrate that our feedforward dual-branch architecture generates versatile and spatially aligned PBR materials suitable for industry-level 3D garment design.

==> section/3.Method_bak.tex <==
\section{Method}
\label{sec:method}

% Describe our method in general (goal + feature)
NI-Tex is designed for image-based garment texture generation with a special enhancement for non-isometric image-garment pairs. In the rest of this section, we first formally define the task of image-based garment texture generation (section~\ref{subsec:ProblemSetting}), then sequentially introduce the key design choices, including Cross-pose Training (section~\ref{subsec:Cross-pose}), Non-isometric Texture Transfer (section~\ref{subsec:Cross-geometry}) and Test Time View Selection (section~\ref{subsec:ViewSelection}). Finally, we elaborate the implementation details in section~\ref{subsec:Training}.

% We propose a new model for the task of image-based garment texture generation. Our model is capable of generating high-quality PBR texture maps for a given garment mesh conditioned on input image prompts. It is robust to variations in the quality and structure~\xiangru{What does quality and structure mean, defined it clearly!} of the input images and does not require strict geometric alignment between the image and the target mesh. Consequently, the image prompt can be either a well-rendered reference image or a masked clothing image obtained from the Internet.

% What did we do to achieve that?
% We first introduce \emph{3D Garment Video} in Section~\ref{subsec:Cross-pose}, enabling the model to learn pose-invariant texture representations and allowing consistent transfer of 2D wild garment appearances onto a canonical garment geometry. We utilize Nano Banana to construct diverse geometries while preserving consistent textures in Section~\ref{subsec:Cross-geometry}, which enhances the model’s ability to transfer textures across different garment geometries. Finally, we design a dual-branch training architecture for PBR texture transfer, as detailed in Section~\ref{subsec:Training}. In addition, we introduce a switchable multi-channel U-Net that accommodates different types of training data and optimization objectives.

\subsection{Problem Setup}
\label{subsec:ProblemSetting}
Image-based garment texture generation takes an input RGB image $I \in \mathbb{R}^{H\times W \times 3}$ and an input geometry represented by a mesh, and output multiple generated texture maps (albedo, roughness, metallic). Each texture map is defined as an image $a\in \mathbb{R}^{N \times N \times C}$ in the UV space of the input geometry. Albedo, roughness, metallic texture map contains $C=3,1,1$ channels, respectively. 
% In 3D garment asset design, high-quality meshes are expensive and labor-intensive to produce, while generative methods often yield coarse, fragmented, and poorly structured meshes. In industrial practice, a few thousand 3D meshes are sufficient to cover nearly all garment categories. In contrast, garment textures exhibit extreme diversity, and billions of wild 2D garment images are readily available online. This suggests that the key challenge is not mesh generation, but effectively associating 2D images with 3D meshes, and developing methods to extract PBR textures from arbitrary garment images and accurately bake them onto standardized industrial garment geometries.

\subsection{Cross-pose Training via 3D Garment Videos}
\label{subsec:Cross-pose}

In this section, we introduce \textbf{3D Garment Videos}, representing garment-centric physical simulation sequences, which can be formulated as,
\begin{equation}
V = \{M_1, M_2, M_3, \dots, M_n\} 
\label{eq:3D videos}
\end{equation}
The geometric deformations of each garment $M_i$ are driven by coherent movements of the wearer. Each video frame is defined by a 3D garment mesh, with a consistent \textbf{albedo} attribute across all frames like Figure~\ref{fig:overview} (Data Space). Moreover, we observe that variations in the specular appearance of fabrics are primarily determined by \textbf{roughness}, while the \textbf{metallic} component is typically negligible. Furthermore, a single garment typically exhibits uniform material properties, indicating that its PBR attributes should not vary significantly across its surface.

We construct our 3D Garment Videos based on the \textbf{BEDLAM}\cite{black2023bedlam} dataset. 
BEDLAM contains nearly 1,700 distinct garment albedo textures, each associated with hundreds of motion sequences, and each sequence consists of hundreds of frames. 
Since the original dataset does not provide roughness or metallic attributes, we augment the selected motion sequences by assigning PBR material properties to each frame. 
Specifically, we set roughness and metallic values as: 
\begin{equation}
\begin{aligned}
\text{roughness} &\sim \mathcal{U}(0,1) \\
\text{metallic} & = 0
\end{aligned}
\end{equation}
We encode roughness and metallic into an RGB image, where the R channel is fixed to 255, and the G and B channels store the corresponding values scaled by 255. For each frame, we randomly apply different types of lighting sources, including point lights, area lights, and environment lights. We render the garment under 10 views, capturing the illumination effects together with material-related attributes (e.g., PBR texture properties) and geometry-related attributes (e.g., normal images and position images).

% \textbf{View Selection.}
% Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready Ready 
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{imgs/demo_for_ViewSelection.pdf}
%     \caption{123}
%     \label{fig:DemoForViewSelect}
% \end{figure}


\textbf{Training Data Stream for Texture Transfer.} From each video, we randomly sample two frames. 
One of them is randomly selected as the \textbf{condition 3D frame}, while the other serves as the \textbf{supervision 3D frame} like Figure~\ref{fig:overview} (Model Training Pipeline). For the condition 3D frame, we randomly choose one rendering image under lighting from a specific viewpoint to obtain the condition image, which is used as the input image prompt. 
In addition, we use its normal and position maps from ten viewpoints as geometric constraints. 
For the supervision 3D frame, we use its PBR texture attributes from ten viewpoints as supervision. Through mutual supervision between frames, the model learns to capture texture variations across different poses during motion, leading to more stable texture transfer. 
Moreover, since 3D garment videos allow bidirectional pairing between any two frames, the training pairs can be formed combinatorially. 
As a result, hundreds of thousands of frames can be expanded into \textbf{tens of billions} of training samples.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{imgs/GraphExplain.pdf}
    \caption{123}
    \label{fig:GraphExp}
\end{figure}

% Graph Figure (Node, Edge)
% Graph Figure
% Graph Figure
% Graph Figure
% Graph Figure

\textbf{MR Rectification.} Since the metallic and roughness materials of frames are different, their reflective behaviors can vary across frames. As a result, directly using the metallic and roughness images from the supervision 3D frame cannot correctly supervise the corresponding attributes of the condition 3D frame. However, because we assign globally consistent metallic and roughness values to each frame, cross-frame attribute transfer becomes straightforward. Specifically, we retrieve a representative foreground pixel value of metallic and roughness from the condition 3D frame and use it to replace the global foreground regions of the supervision 3D frame, enabling consistent supervision during training.

% MR Rectification Figure
% MR Rectification Figure
% MR Rectification Figure
% MR Rectification Figure
% MR Rectification Figure

\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/demo_for_MR_Rec.pdf}
    \caption{123}
    \label{fig:MRRexDemo}
\end{figure}

\subsection{Non-isometric Texture Generation via }
\label{subsec:Cross-geometry}
When texture transfer is performed from an input wild image, garments are often partially occluded by human poses or other objects, leading to information loss. 
Moreover, our goal for the model is to bridge the geometric gap between different types of garments, allowing texture extraction and transfer across diverse geometries. For example, transferring textures from skirts or shorts onto the geometry of long pants.

Therefore, we randomly select rendered views of frames from the 3D garment videos and apply \textbf{Nano Banana} to modify their geometries while preserving the original textures. We choose to use the illuminated renderings rather than the albedo images, as this allows Nano Banana to generate results that are more consistent with real-world appearances and helps reduce the inference-stage domain gap. The modified images are used to replace the original condition images, while supervision is still provided by the original supervision 3D frames. Through such cross-category training, we effectively distill texture identity consistency from Nano Banana.

% Nano Banana Results Figure
% Nano Banana Results Figure
% Nano Banana Results Figure
% Nano Banana Results Figure
% Nano Banana Results Figure
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{imgs/DemoForNB.pdf}
    \caption{123}
    \label{fig:NBDemo}
\end{figure}

When modifying the garment geometries, it is essential to preserve the semantic consistency of the textures to avoid incorrect distillation from Nano Banana. 
We follow three key principles to ensure semantic stability.

\begin{enumerate}
    \item \textbf{Category-wise texture consistency.} When altering the geometry of full-body garments, we ensure that textures of the upper and lower garments (e.g., tops and skirts or pants) do not drift or swap incorrectly.
    \item \textbf{Inner–outer texture consistency.} When modifying layered outfits, we ensure that the textures of outer garments are not confused with those of inner garments.
    \item \textbf{Allowance for additional human body or accessory generations.} We allow Nano Banana to occasionally generate extra human parts or accessories, which helps the model focus more robustly on garment materials and automatically ignore irrelevant or mistakenly masked regions in wild images.
\end{enumerate}

\subsection{Test Time View Selection}
\label{subsec:ViewSelection}

\subsection{PBR Texture Transfer Training}
\label{subsec:Training}
To preserve the texture information from the input image prompt during training, we adopt a \textbf{feedforward dual-branch architecture} composed of a \textbf{guidance branch} and a \textbf{training branch} like Hunyuan3D \cite{hunyuan3d2025hunyuan3d}, both implemented with identical U-Net backbones. The guidance branch extracts hierarchical features from the input image and feeds them into the corresponding layers of the training branch as reference information. The training branch takes multi-view normal and position maps as input to enforce geometric and 3D consistency, while leveraging the reference features to perform multi-channel inference of albedo and MR (metallic and roughness) attributes.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{imgs/Model Architecture.pdf}
    \caption{123}
    \label{fig:ModelArchitecture}
\end{figure}

 \subsubsection{Switchable Multi-Channel U-Net}
 We adopt the \textbf{Multi-Channel Aligned Attention (MCAA)} module from MaterialMVP \cite{he2025materialmvp} to connect the two branches. 
As defined in Equation (\ref{eq:MCAA}), we extract the reference texture features from the guidance branch and inject them into the albedo channel of the training branch:
\begin{equation}
\text{Attn}_{albedo} = \text{Softmax}\left( \frac{Q_{albedo} K_{ref}^{T}}{\sqrt{d}} \right) \cdot V_{ref}
\label{eq:MCAA}
\end{equation}

To achieve spatial and geometric alignment between the MR and albedo attributes, we inject the albedo attention into the MR latent representation:
\begin{equation}
z_{MR}^{new} = z_{MR} + \text{Attn}_{albedo},
\label{eq:MR-Aligned}
\end{equation}

In 3D garment videos, the MR attributes are accurately rectified, allowing the MCAA module to synchronize and generate well-aligned material properties. 
However, images generated by Nano Banana often exhibit inconsistent surface reflections, making it unnecessary to optimize their MR attributes during training. To address this, we introduce the \textbf{switchable multi-channel U-Net}, where the MR channel can be deactivated when only albedo optimization is required, thereby improving training efficiency.


\subsubsection{Training Strategy}
Since the MR values in our 3D garment videos are globally uniform, the model tends to overfit these constant properties during training. To enhance the network’s perception and generalization across diverse MR materials, we incorporate additional supervision from the \textbf{Objaverse} and \textbf{TexVerse} datasets for mixed training.

The model $\epsilon_{\theta}$ generates two diffusion noises $\epsilon_{t}^{MR}$ and $\epsilon_{t}^{MR}$ conditioned on the input image $I$ at training timestep $t$. In the multi-channel optimization stage, loss can be designed as:
\begin{equation}
 \mathcal{L}{_\text{1}}=\mathbb{E}_{\epsilon\sim\mathcal{N}(0,1),\,t}\left[\left\|\epsilon-\epsilon_{t}^{MR}\right\|_{2}^{2}+\left\|\epsilon-\epsilon_{t}^{Albedo}\right\|_{2}^{2}\right]
\end{equation}
When the switchable multi-channel U-Net deactivates the MR channel, the optimization is performed solely on the albedo channel:
\begin{equation}
 \mathcal{L}{_\text{2}}=\mathbb{E}_{\epsilon\sim\mathcal{N}(0,1),\,t}\left[\alpha*\left\|\epsilon-\epsilon_{t}^{Albedo}\right\|_{2}^{2}\right]
\end{equation}
To alternately optimize $\mathcal{L}{_\text{1}}$ and $\mathcal{L}{_\text{2}}$, we set the balancing factor $\alpha = 2$ to smooth the loss curve during training.

